Optimal Interpolation and Prediction in Pulsar Timing

For pulsar projects it is often necessary to predict the pulse phase in advance, for example, when preparing for new observations. Interpolation of the pulse phase between existing measurements is also often required, for example, when folding X-ray or gamma-ray observations according to the radio pulse phase. Until now these procedures have been done using various ad hoc methods. The purpose of this paper is to show how to interpolate or predict the pulse phase optimally using statistical models of the various noise processes and the phase measurement uncertainty.

==> PaxHeader/resubmit.tex <==
14 gid=286816
20 ctime=1335506177
20 atime=1335506177
38 LIBARCHIVE.creationtime=1334725865
24 SCHILY.dev=234881026
23 SCHILY.ino=10128228
18 SCHILY.nlink=1


==> response.tex <==
Response to referee
----------------------------


We thank the referee for the many constructive comments on our paper.  We have addressed all the issues raised and have followed the referee's advice on nearly all points.  These are detailed below.

1 - INTRODUCTION:

Paragraph 1:

"predicted precisely"
--> "precisely predicted"

Done


"with the prediction of the timing model ... using a least squares procedure, ..."
--> "with the prediction of a timing model, whose parameters are adjusted using a least-squares procedure, ..."

Done

"... during the first discovery ..."
--> "... with the discovery ..."

Done

"... known as the "residuals".  Ideally, the residuals would simply reflect the measurement uncertainty, but ..."
--> "... known as "timing residuals".  Ideally, these residuals would simply reflect the ToA measurement uncertainty, but ....

Done

"..., or the interplanetary medium (...), or even ..."
--> "..., the interplanetary medium (...), or even ..."

Done


Paragraph 2:

* FITWAVES: is there a reference of some kind for this?

Done

"... obtaining a simple, ..."
--> "... obtaining and using a simple, ..."

Done

"... of the timing noise and using that model to calculate ..."
--> "... of the timing noise in order to calculate ..."

Done

"... we will discuss below."
--> "we will discuss in the following section."

Done

Paragraph 3:

"... necessary to sum individual pulses for the duration of the observations."
--> "... necessary to sum many individual pulses during the observations."

Done

"... then "folding" the gamma-ray photons according to this model."
--> "... then "folding" the gamma-ray photons into the predicted phase bin." (or something like this)

Done

"However, as shown below, ..."
--> "However, as we demonstrate in subsequent sections, ..."

Done


Paragraph 4:

"Typically this is carried out ..."
--> "This is typically carried out ..."

Done

* Perhaps is is more accurate to say "the extrapolated timing model is typically described in tempo2 using a Chebyshev polynomial expansion..." ?

This was not changed.  Tempo2 uses a complete timing model for the pulsar and, internally, does not use Chebyshev polynomials.  In order to create a simple model for observing hardware, tempo2 does have the option to output the model as Chebyshev polynomials, but tempo2 itself does not use this approximation.

* The portion about the space navigation applications (starting with "It is hoped...") should probably be a separate paragraph, and for flow's sake, perhaps introduce with something like, "An example of a practical use of..."

Done


Paragraph 5:

"... and use the real data for PSR J1939+2134 ..."
--> "... and use real data from observations of PSR J1939+2134 ..."

Done

2 - THE MAXIMUM LIKELIHOOD FILTER

This is generally well-explained!

Paragraph 1:

"... and the algorithm has become ..."
--> "... and the corresponding algorithm has become ..."

Done

"However Wiener filters ..."
--> "However, Wiener filters ..."

Done

"Effectively this is ..."
--> "This is effectively ..."


Done

Paragraph 2:

"the log "
--> "the logarithm"

Done

Paragraph 3:

"premultiply"
--> "pre-multiply" (I think!)

Done

Paragraph 4:

* "... with zero terms on the diagonal corresponding ..."
--> "... with terms of value zero along the diagonal, corresponding ..."

Done

3 - TESTING THE ALGORITHM

Paragraph 1:

* As I understand, you have used the 1713 data for its sampling and ToA uncertainties only, and generated your own data set of timing residuals at those samples, with the 1713 uncertainties.  If I am correct, perhaps some of the following suggestions would make things a bit clearer:

* "With this sampling, we simulated red noise and added white noise to each observation."
--> "With this sampling, we simulated a data set of timing residuals with red noise, and added white noise to these generated observations."

Done.  The referee is correct.


* It would be nice to describe each component variable of your equation for P(f) here, since you refer to A, f_c, and alpha multiple times throughout.

Done

* Just to clarify, are you using alpha=4.3, or the exact value of 13/3 = 4.3333333... ?  If it's the latter, please say so.  It would be good to quickly show where this power spectrum comes from, in terms of the strain spectrum with power-law exponent -2/3, as this is what people are most familiar with.

Done.  We used 4.3333 and made this clearer in the text.


* "... are shown in Figure 3" -- do you mean Figure 1?

Done -- the referee is correct.  That was a latex issue!

"... caused by rotational irregularities, ..."
--> "... caused by unexplained rotational irregularities, ..." (to contrast with explained irregularities, such as glitches, which you mention next)

Done


Paragraph 2:

* It is unclear why you created one long data set 50x longer than your data length and split it up, versus creating 50 data sets.  Are each of these 50 realisations including the +/- 5000 days tacked on to each end?  Explain briefly.

Done.  This has been improved.

* Why did you not add white noise to the regularly-spaced samples?

Done.  This has been explained in the text.

Paragraph 3:

"... covariance functions from the data, instead ..."
--> "... covariance functions from the data; instead ..."

Done

* "Error bars representing the white noise level are overlaid."
--> "Error bars representing the white noise level are overlaid, at the locations of the sampled data points."

Done

* To make things clearer, perhaps it would be best to group the statement that the interpolation works well, with the evidence for this -- namely that the discrepencies are less than the white noise level used, and place the above description of the white noise error bars further up, with the description of Figure 2.

We have modified the structure of this section slightly.

* You mention that the extrapolated function converges to the timing model prediction twice here, once after your statement that the interpolation works well, and then at the end of the paragraph.  I would suggest making all the statements regarding the interpolation results, then move on to those of the extrapolation, to keep a clear flow.

As above.

4 - APPLICATIONS

4.1 - Timing noise modelling and removal

Paragraph 1:

"... and the post-fit residuals (after removing this model) are shown ..."
--> "... and these post-fit residuals, once this model is removed, are shown ..."  (The fact you remove the model should probably not be in parentheses, as it is an important point.)

Done

Paragraph 2:

* You say that the residuals are significantly whiter than those from applying FITWAVES, but you should perhaps quantify this comparison.

We have changed this section as testing for ``whiteness'' is not trivial.  Now we simply say that the rms of the discrepancies is smaller.


Paragraph 3:

* "... provides a reasonable interpolation during the data gap."
--> "... provides an interpolation that more closely represents the original observations during the data gap."

Done


4.2 - Spacecraft navigation

Paragraph 1:

In addition to your existing references, perhaps also include proceedings by Bernhardt et al. 2010/2011 (arXiv:1011.5095/1111.1138)

Done

5 - DISCUSSION

5.1 - Glitch events

Paragraph 1:

* "For instance, if possible, the glitch event should be modelled and its parameters included in the pulsar timing model."  This just repeats the previous sentence, and so should probably be removed.


Done

Paragraph 2:

* "100 ns of white noise"
--> "white noise with rms of 100 ns".  Also, why are you choosing 100 ns?  Is it simply to have "typical" error bars?  Explain.

Done.  The 100ns is not very important - it simply allows us to demonstrate the effect of a glitch that is larger than the white noise level.

* "For this data set the interpolation procedure correctly models the timing residuals."
--> "The difference between the interpolated timing residuals and the this data set is less than the white noise level, demonstrating ..."  (or something like this)

Done

5.2 - Sensitivity to errors in the parametrisation of the noise

Paragraph 1:

"... to be interpolated or extrapolated."
--> "... to be modelled by interpolation or extrapolation."


Done

Paragraph 2:

* This is laid out really nicely!  The one thing I would clarify would be in describing how you rotate incorrect values of the parameters alpha, f_c, and sigma_w^2.  For example, as you vary parameters by offsetting them from the correct value, do you vary one parameter while holding the others fixed at the correct values?  This is important to distinguish for interpreting Figure 6.  It would be good to outline the magnitude of the changes in your "incorrect trials" in the main text, as opposed to only in the figure caption.

Done.  We held the other parameters fixed. This is clearer now in the text

"... as three lines ..."
--> "... as the three lines ..."

Done


Paragraph 3:

* Could you describe the how "significantly smaller" the discrepencies are than the white noise? (e.g. a factor of ... / ... orders of magnitude)

The text has now been updated to make this clearer.  

* "... after the quadratic polynomial removal."
-->"... after the quadratic polynomial removal (see next section)."

We did not make this change as the next section does not specifically deal with the sensitivity to parameter errors.

* "... the duration for which timing residuals can be extrapolated is reduced when compared ..."  Reduced by how much (e.g. a factor of...)

We haven't done any quantitive analyses, but hopefully this makes more sense now.  It's very hard to do this in more detail as it depends on the red noise, white noise, error in the parameters and how much the user is happy with small errors in the extrapolation.  We've tried to make this clearer in the text.

* "... smaller tha variations in the different realisations ..." How much smaller?

As above

* "The technique is therefore insensitive to errors in the model parameters ..." This doesn't really give a sense of how large these errors can be while the technique remains insensitive.  Is there something that can be said about this?  For example, if there are errors that are large enough to render the technique more sensitive, could the magnitude of those errors be considered realistic or not?

As above

5.3 - Quadratic removal of the timing noise

Paragraph 2:

"... converge to the timing models. As these ..."
--> "... converge to the timing models; however, as these ..."

Done

"The exact method for ..."
--> "The exact method in this case for ..."

Done

FIGURES:

Figure 2:

* - Make dotted line more visible
- probably "(back)" not needed since you say it is for 5000 d before and after

Done

Figure 3:

* - You haven't defined what is meant by "strongest", "intermediate-level", or "weakest" red noise.  Perhaps, along with the definitions of the three spectral densities in Figure 1, define these in the main text?

Done

* - perhaps move the sentence "The rms of these realisations..." down to appear just before the sentence "The rms difference between ...", for clarity.

Done


Figure 4:

* "The lower part contains ..."
--> "The lower part of each panel shows ..."

Done


Figure 5:

* - explain error bars on lower panel.

Done

- Perhaps adjust units on top panel vertical axis to be in microseconds instead of seconds?

Done

Figure 6:

- This is a nice, demonstrative plot.

* "... sensitivity to the spectral component error alpha, ..."
--> "... sensitivity to changes in the spectral component alpha"
- and similarly for the next two parameters, removing possible confusion between the name of the parameter versus parameter error.


* - Could make more concise by saying something like, "The dotted, dashed, and solid lines show the sensitivity to errors in the parametrisation of the spectral component alpha, corner frequency f_c, and the white noise sigma_w^2, respectively. These are represented on the horizontal axis by alpha-alpha_0, log_10(..), ..."
(This also avoids confusion between the words "error" vs. "uncertainty" in this case).

Done



Figure 7:

- Perhaps ms would be better vertical axis units for the top panels?

Done


* "The left-handed panel shows the residuals ..."
--> "The left-handed top panel shows ..."

Done


* "The right-handed panel ..."
--> "The right-handed top panel ..."

Done


* There is no mention or description here of the dotted line, which should precede the final sentence about the bottom panels.

Done


"... actual residuals and the interpolated function."
--> "... residuals and the interpolated function during the data span."

Done



Figure 8:

* "The difference between ..."
--> "Top:  the difference between ...", or "the top panel shows ...", or something of this kind.

Done


* "... given two models for PSR J1939+2134."
--> "... given the two models for PSR J1939+2134, shown in Figure 7."

Done


"The lower panel is a zoom-in ..."
--> "Bottom: a zoom-in ..."

Done

